Self-Supervision & Meta-Learning for One-Shot Unsupervised Cross-Domain Detection

Deep detection approaches are powerful in controlled conditions, but appear brittle and fail when source models are used off-the-shelf on unseen domains. Most of the existing works on domain adaptation simplify the setting and access jointly both a large source dataset and a sizable amount of target samples. However this scenario is unrealistic in many practical cases as when monitoring image feeds from social media: only a pretrained source model is available and every target image uploaded by the users belongs to a different domain not foreseen during training. We address this challenging setting by presenting an object detection algorithm able to exploit a pre-trained source model and perform unsupervised adaptation by using only one target sample seen at test time. Our multi-task architecture includes a self-supervised branch that we exploit to meta-train the whole model with single-sample cross-domain episodes, and prepare to the test condition. At deployment time the self-supervised task is iteratively solved on any incoming sample to one-shot adapt on it. We introduce a new dataset of social media image feeds and present a thorough benchmark with the most recent cross-domain detection methods showing the advantages of our approach.

==> implement.tex <==
We built our model over a public implementation of Faster-RCNN \cite{massa2018mrcnn}. Specifically we chose a ResNet-50 \cite{he2016deep} backbone pre-trained on ImageNet, RPN with 300 top proposals after non-maximum-supression, anchors at three scales (128, 256, 512) and three aspect ratios (1:1, 1:2, 2:1).

In the following, we will differentiate the name of the proposed model, depending on the specific adopted training procedure. We will indicate with OSHOT our basic One-SHOT multi-task pretrained approach, while we will use FULL-OSHOT to refer to the variant based on meta-learning pretraining. 
We also consider two intermediate cases: \emph{Tran}-OSHOT extending OSHOT with the data semantic-preserving transformations used in FULL-OSHOT, and \emph{Meta}-OSHOT that corresponds to FULL-OSHOT without transformations (\ie $K=1$). 

For OSHOT we train the base network for 70k iterations using SGD with momentum set at $0.9$, the initial learning rate is $0.001$ and decays after 50k iterations. We use a batch size of 1, keep batch normalization layers fixed for both pretraining and adaptation phases and freeze the first 2 blocks of ResNet50. The weight of the rotation task is set to $\lambda=0.05$.
%
FULL-OSHOT is actually trained in two steps. For the first 60k iterations the training is identical to that of OSHOT, while in the last 10k iterations the meta-learning procedure is activated. The inner loop optimization on the self-supervised task runs with $\eta=5$ iterations and the batch size is 2 to accomodate for two transformations of the original image. Specifically we used gray-scale and color-jitter with brightness, contrast, saturation and hue all set to $0.4$. All the other hyperparameters remain unchanged as in OSHOT.
%
\emph{Tran}-OSHOT differs from OSHOT only for the last 10k learning iterations, where the batch size is 2 and the network sees multiple images with different visual appearance in one iteration. \emph{Meta}-OSHOT is instead identical to FULL-OSHOT, made exception for the transformations which are dropped, thus the batch size is 1 also in the last 10k pretraining iterations. 

The adaptation phase is the same for all the variants: the model obtained from the pretraining phase is updated via fine-tuning of the self-supervised task. The batch size is equal to 1 and a dropout with probability $p$ = 0.5 is added before the rotation classifier to prevent overfitting. The weight of the auxiliary task is increased to $\lambda$ = 0.2 to speed up the adaptation process. All the other hyperparameters and settings are the same used during the pretraining. The number of fine-tuning steps is set to match the number of iterations in meta-training $\gamma=\eta=5$, but we also investigated the effect of increasing $\gamma$ for OSHOT (see Section \ref{sec:increasingiter}).
%The official total number of fine-tuning steps on the single target image is 30, but for our experiments we use 10 as maximum number of steps, because we want to show that with our procedure the network is already able to achieve better results in fewer iterations.
